State-Space Identification of Unmanned Helicopter Dynamics using Invasive Weed Optimization Algorithm on Flight Data

In order to achieve a good level of autonomy in unmanned helicopters, an accurate replication of vehicle dynamics is required, which is achievable through precise mathematical modeling. This paper aims to identify a parametric state-space system for an unmanned helicopter to a good level of accuracy using Invasive Weed Optimization (IWO) algorithm. The flight data of Align TREX 550 flybarless helicopter is used in the identification process. The rigid-body dynamics of the helicopter is modeled in a state-space form that has 40 parameters, which serve as control variables for the IWO algorithm. The results after 1000 iterations were compared with the traditionally used Prediction Error Minimization (PEM) method and also with Genetic Algorithm (GA), which serve as references. Results show a better level of correlation between the actual and estimated responses of the system identified using IWO to that of PEM and GA.

==> README <==
%% ahsmeeting.sty and ahs.bst README file
%
% This work consists of the files ahsmeeting.sty and ahs.bst.
%
% Copyright 2014 Matt Floros
% Release 1.16, June 10, 2014
% Copyright notice:
% This package consists of the files ahsmeeting.sty and ahs.bst.
% Permission is granted to use, distribute, modify, and create derivative works
% from this package subject to the following conditions:
% 
% User agrees that the package is provided 'as is,' without warranty of any
% kind, either expressed or implied, including, but not limited to, the implied
% warranties of merchantability and fitness for a particular purpose.  User
% assumes all risk and responsibility for ensuring that it works as desired. 
% No user should expect, and no derivative work should imply that any support
% is provided by the author.
%
% Modified versions and derivative works must contain a summary of changes, and
% information written to the screen and in comments should clearly state that
% it is a modified version and who the last person to modify the package is.

This package provides LaTeX and BibTeX style files for AHS International
(formerly the American Helicopter Society) meeting proceedings.  It is current
as of the Author Guide for AHS Forum 71 (2015).

Included Files:
README (this file)
ahsmeeting.cls (LaTeX document class)
ahsmeeting.sty (LaTeX style file)
ahs.bst (BibTeX style file)
manual.tex (source for PDF manual)
manual.pdf (manual for style files)
template.tex (source for paper template--should be processed with pdflatex)
abstract.tex (source for abstract template--should be processed with pdflatex)
template.pdf (paper template which matches MS Word template)
abstract.pdf (abstract template which matches MS Word template)
40x80.jpg (image of LRTA in wind tunnel for template document)

Required Packages:
cite.sty
times.sty
helvet.sty
mathptmx.sty
ifthen.sty

Features:

In general the philosophy taken was to conform to specific formatting guidelines
in author guide for the current annual meeting.  Formatting beyond that is
selected to mimic the Journal of the American Helicopter Society.  Specific
formatting includes

 - Margins
 - Page number centered at the bottom (New starting in 2012)
 - Abstract centered across entire first page
 - Meeting and copyright footnote
 - Section headings
 - Citation labels
 - Alphabetic footnotes in tables
 - Formatting of references
 
Package Options:
 draft
     Places box at top of every page indicating draft and the date and time the
     document was processed.
 plaincite
     Passed directly to cite package to remove citation labels.  See cite
     package documentation for details.
 SECTION 
     Places section headings (\section only, not \subsection and down) in all
     caps
 absheading
     Places word "Abstract" above abstract on title page, in caps if SECTION
     option is also used.
 jahsabs
     Causes abstract block to be bold like the Journal of the American
     Helicopter Society. 
 plainabs
     Causes abstract block to be normal typeface. (default)
 bigtitle
     Increases font sizes for title and author blocks (\Large and \large)
 smalltitle
     Decreases font sizes for title and author blocks (\large and \normalsize)
 bigsection
     Increases font size for main section headings (\large)
 smallsection
     Normal font size for main section headings (\normalsize)

Command Summary:
 \meeting{text}
     This makes a footnote at the beginning of the first page for  the name of
     the meeting and copyright info.  There is no indentation and no footnote
     mark per AHS guidelines

 \nomeeting
     This command removes the source footnote entirely.  It is intended to be
     used when writing abstracts which do not require a source footnote.

 \abstract{text}
     This places the abstract below the title/author block, but makes it bold,
     6.5" wide (default text width is 7in), centered, and single column per AHS
     guidelines.  Must be issued before \maketitle command.

 \draft
     Ripped from a Penn State thesis style file (which in turn was apparently
     ripped from cwebmac.tex), this places a centered box at the top of each
     page with the date and time and the word "draft." Also available as a style
     option.
    
 \symbolentry{symbol}{definition} 
     Creates an entry where a the first argument is a mathematical symbol and
     the second is its definition.  Note that the mathematical symbol is
     automatically typeset in math mode, so the \mbox command must be used if
     the symbol is to be plain text.  The definition can be several lines and
     will automatically be wrapped to subsequent lines if it is too long for a
     single line.

 \setsymbolwidth{width}
     Sets the width of the symbol in the notation.  If the symbol is longer
     than the set width (for example a coordinate system with several
     components), it will be wrapped.  The definition width is automatically
     adjusted to be the remainder of the column.  The default is 0.5 inches.
     
 \singleauthor[width]{author}
     Sets an author entry inside a parbox of specified width (default 2in).  It
     can be used to tweak spacing between authors.

 \doubleauthor[width]{author1}{author2}{common}
     Typesets two authors with some unique information and some common
     information.  The unique information is placed below each author and the
     common information is centered below both authors.  Within each argument,
     lines are broken with \\ as normal.  The optional argument [width] can be
     used to specify the width each author should use; the common information
     can be 2*width wide.  Default width is 2in.

 \tripleauthor[width]{author1}{author2}{author3}{common}
     Typesets three authors with some unique information and some common
     information.  The unique information is placed below each author and the
     common information is centered below the three authors.  Within each
     argument, lines are broken with \\ as normal.  The optional argument
     [width] can be used to specify the width each author should use; the common
     information can be 3*width wide.  Default width is 2in.

 \quadauthor[width]{author1}{author2}{author3}{author4}{common}
     Typesets four authors with some unique information and some common
     information.  The unique information is placed below each author and the
     common information is centered below the four authors.  Within each
     argument, lines are broken with \\ as normal.  The optional argument
     [width] can be used to specify the width each author should use; the common
     information can be 4*width wide.  Default width is 1.5in.

 \andnewline
     Similar to \and when entering author information only forces a new line to
     improve author grouping.

 \footnotedefs (environment)
    Results in smaller text and spacing for footnotes within tables.  It is
    recommended to enclose tables in a minipage environment and use the LaTeX
    standard footnote commands if possible.  \footnotedefs should only be needed
    if a footnote in the table caption is needed.   

 \appendix
    Starts appendix.  The style file can automatically count appendices (based
    on lastpage.sty) so that a single is labeled "Appendix" and multiple are
    labeled "Appendix A", "Appendix B," etc. User can use \label and \ref to
    reference multiple appendices.  Note: If only one appendix is present, 
    using \section{Appendix} will achieve the same thing as \appendix.  

